Designing the Business Conversation Corpus

While the progress of machine translation of written text has come far in the past several years thanks to the increasing availability of parallel corpora and corpora-based training technologies, automatic translation of spoken text and dialogues remains challenging even for modern systems. In this paper, we aim to boost the machine translation quality of conversational texts by introducing a newly constructed Japanese-English business conversation parallel corpus. A detailed analysis of the corpus is provided along with challenging examples for automatic translation. We also experiment with adding the corpus in a machine translation training scenario and show how the resulting system benefits from its use.

==> REVIEWS.tex <==
============================================================================
                            REVIEWER #1
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 3
      Originality / Innovativeness (1-5): 3
           Soundness / Correctness (1-5): 2
             Meaningful Comparison (1-5): 2
                      Thoroughness (1-5): 2
        Impact of Ideas or Results (1-5): 2
                    Recommendation (1-5): 3
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
<p> This paper introduced a new Japanese-English parallel corpus of business conversation and analyzed it from the viewpoint of zero
anaphora.  In addition, the authors analyzed translation quality and examples translated by SMT and NMT systems based on this corpus.

<p> 1) The reviewer recognizes that the corpus is original.  However, the analyses and the translation experiments are incomplete.
<p> First, the authors analyzed the corpus from the viewpoint of zero anaphora.  To my knowledge, many researchers classify the anaphora into three types; intra-sentential, inter-sentential, and exophoric relations [Iida+ 2007].  Among them, the intra-sentential relation is not a problem because the antecedent exists in the sentence.  This paper is unclear about this classification.
<p> Moreover, some zero-pronouns can be automatically complemented using modality expressions and/or domain information even if the antecedents are not in the sentence.  Anaphora types that affect to translation quality should be factorized.
<p> Anaphora and context dependent translation are both difficult problems.  However, at least to say, the authors should distinguish three anaphora types for discussing context dependent translation.

<p> 2) Although the authors trained 1-to-1 MT systems, 2-to-2 translation can be realized using existing MT systems [Tiedemann and Scherrer 2017].  It is better to exploit 2-to-2 translation because the characteristic of the corpus is to maintain context information.

<p> Detailed comments are as follows:

<p> 3) Sec. 1 (p.1, line 086) and Sec. 4 (p.4, line 395)
<br> 30,000 sentences are too small for training of NMT systems.  Rather, it is better to use the corpus for evaluation and domain adaptation.

<p> 4) Table 2 (p.2), Sec. 2.1 (p.2, line 196)
<br> In dialogue processing, a dialogue is roughly classified into a task-oriented one or a chat.  Are the collected conversations distinguishable between two types?

<p> 5) Sec. 2 (p.2, line 186)
<br> Does the second condition mean that writers are bilingual?  If so, this condition seems to be tight, and it may be difficult to build large corpora.  Are there any suggestions for creating large corpora?

<p> 6) Sec. 2.2 (p.3, line 206)
<br> Usually, translation quality depends on a translation direction.  It might be good that the corpus contains conversations of the both directions in the same amount.

<p> 7) Sec. 3 (p.3, footnote 5)
<br> It is better to write the version (or the year-month information) of Google Translate.

<p> 8) Sec. 3.1 (p.3, line 278)
<br> This is an example of the intra-sentential relation, but it might not be suitable here because the antecedent of the intra-sentential relation can be complemented from the sentence.  The inter-sentential relation is suitable for the purpose of the corpus.

<p> 9) Sec. 3.3, the first paragraph (p.4, line 340)
<br> This is an example of the inter-sentential relation, not the exophoric relation.

<p> 10) Sec. 3.3, the 2nd paragraph (p.4, line 376)
<br> This is an example of the exophoric relation, but the speaker can be inferred from the modality expression in the sentence.

<p> 11) Table 3
<br> This time, the authors used dialogue data as the out-of-domain corpora.  However, it becomes difficult to increase the amount if the data is restricted to dialogues.  The reviewer thinks that written parallel corpora can be used as the out-of-domain data.

<p> 12) Sec. 4.1 (p.5, line 423)
<br> Please describe the English tokenizer for the evaluation.

<p> 13) Table 5 (p.5)
<br> The reviewer did not understand what was found from this table.  If the authors want to indicate that the models had not been overfitted, please explain what values indicate the overfitting.

<p> 14) Figure 5 (p.6)
<br> The order of Reference, Our Best NMT, and Google Translate should be coordinated with the other figures.

<p> 15) Sec. 5 (line 567)
<br> The reviewer recommends performing experiments of context translation early.

<p> [Iida+ 2017]
@InProceedings{iida-EtAl:2007:LAW,
  author    = {Iida, Ryu  and  Komachi, Mamoru  and  Inui, Kentaro  and  Matsumoto, Yuji},
  title     = {Annotating a Japanese Text Corpus with Predicate-Argument and Coreference Relations},
  booktitle = {Proceedings of the Linguistic Annotation Workshop},
  month     = {June},
  year      = {2007},
  address   = {Prague, Czech Republic},
  publisher = {Association for Computational Linguistics},
  pages     = {132--139},
  url       = {http://www.aclweb.org/anthology/W/W07/W07-1522}
}
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #2
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 5
      Originality / Innovativeness (1-5): 3
           Soundness / Correctness (1-5): 5
             Meaningful Comparison (1-5): 5
                      Thoroughness (1-5): 4
        Impact of Ideas or Results (1-5): 5
                    Recommendation (1-5): 5
               Reviewer Confidence (1-5): 5

Detailed Comments
---------------------------------------------------------------------------
Spoken language translation is definitely one of the most important direction for MT. The lack of good data is the biggest problem. I believe this new corpus (supposed to be released soon) will be a great contribution to MT research community.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #3
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 5
      Originality / Innovativeness (1-5): 4
           Soundness / Correctness (1-5): 4
             Meaningful Comparison (1-5): 5
                      Thoroughness (1-5): 5
        Impact of Ideas or Results (1-5): 5
                    Recommendation (1-5): 5
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
This paper presents a new dataset on business conversations for EN<->JA


Strength
====

 - This is an interesting mix in corpus representation, i.e. "meetings and negotiations, as well as so-called water-cooler chats" =)
 - Solid examples of 'zero anaphora' in section 3.3
 - Comparative results in NMT and SMT not just on the newly proposed corpus but also on existing similar corpora (translated into Japanese)
 - Good observation the limitation of sentence level MT where it is necessary for document level NMT to resolve some zero anaphora issues


Weakness
====

 - Nothing much. Very well written resource paper!!

Question
====

 - Will this resource/corpus together with the translated AIM and ON corpora be released? 
 - Can this be a new task for next year's WAT? This would be an excellent "challenge set" corpus to test on document-level NMT for next year's WAT


Suggestion
====

- "Zero Anaphora" in the case of pronoun is also known as "pronoun dropping" / "pro-drop" but "zero anaphora" can refer to arguments/entities beyond pronoun. Maybe it'll be good to show another example that is not just pro-drop but argument/entities dropping.
---------------------------------------------------------------------------
